SCOD: From Heuristics to Theory

This paper addresses the problem of designing reliable prediction models that abstain from predictions when faced with uncertain or out-of-distribution samples - a recently proposed problem known as Selective Classification in the presence of Out-of-Distribution data (SCOD). We make three key contributions to SCOD. Firstly, we demonstrate that the optimal SCOD strategy involves a Bayes classifier for in-distribution (ID) data and a selector represented as a stochastic linear classifier in a 2D space, using i) the conditional risk of the ID classifier, and ii) the likelihood ratio of ID and out-of-distribution (OOD) data as input. This contrasts with suboptimal strategies from current OOD detection methods and the Softmax Information Retaining Combination (SIRC), specifically developed for SCOD. Secondly, we establish that in a distribution-free setting, the SCOD problem is not Probably Approximately Correct learnable when relying solely on an ID data sample. Third, we introduce POSCOD, a simple method for learning a plugin estimate of the optimal SCOD strategy from both an ID data sample and an unlabeled mixture of ID and OOD data. Our empirical results confirm the theoretical findings and demonstrate that our proposed method, POSCOD, out performs existing OOD methods in effectively addressing the SCOD problem.

==> X_rebuttal.tex <==
\clearpage
\twocolumn
\pagenumbering{gobble}
\thispagestyle{empty}
\appendix
\setlength{\parskip}{-6pt}
\maketitlerebuttal

\noindent We appreciate the valuable feedback from reviewers  {\bf\color{review1}R1:p7P6}, {\bf\color{review2}R2:8SES}, 
{\bf\color{review3}R3:oWKL}, 
{\bf\color{review4}R4:BgPj}, and 
{\bf\color{review5}R5:kDiA}. In response to their insightful comments, we will incorporate the provided feedback. We apologize for not addressing all of the comments here; we are limited by space constraints.

\boldparagraph{Formulation}
\hspace{-0.5em}\revone has raised concerns regarding the formulation of the SCOD problem (\Cref{def:SCOD}). The suggestion is to substitute the constraint on $\tpr$ with a constraint on coverage. Both formulations are valid; coverage constraint can be found in \cite{Narasimhan-Plugin-Arxiv2023}. While coverage can be determined at test-time, the threshold $\lambda$ (see \cref{thm:SingleCostModel}) can be tuned using validation data and then fixed. Therefore, accessing $\tpr$ at test time is not necessary. In the paper, we show several advantages of constraining $\tpr$:
\begin{enumerate*}[label=(\roman*),before=\unskip{ }, itemjoin={{, }}, itemjoin*={{, and }}]
    \item The problem definition becomes independent of the prior $\pi_O$; hence the optimal solution is independent of prior
    \item constraining $\tpr$ enables the explicit formulation of the optimal score, \cref{equ:optScore}. In contrast, the coverage-based formulation necessitates solving an optimization task to find the mixing coefficient for $r(x)$ and $g(x)$, see \cite{Narasimhan-Plugin-Arxiv2023}
    \item constraining $\tpr$ aligns with the task's goal; practitioners are likely to prefer accepting a specific portion of ID rather than of all samples.
\end{enumerate*}

\boldparagraph{PAC Learnability \& PLOSCOD}
\hspace{-0.5em}%By \textit{"distribution-free setup"} we refer to PAC learnability without making assumptions about data distributions. PLOSCOD doesn't claim to solve the SCOD problem without assumptions on distributions. %For instance, in \cref{thm:CorrectedSigmoid}, we assume the existence of a feature map $\phi(x)$. 
\revone and \revthree question the learnability of SCOD. If OOD samples are unattainable, and only ID samples are accessible, SCOD is \textit{not} PAC learnable, as explained in \cref{sec:pac_learnability}. % I.e., when only ID samples are accessible, the task can not be solved without making additional assumptions about the OOD data. 
In \cref{sec:plugin_estimate_of_optimal_scod}, we relax the need for clean OOD samples by assuming a sample from a mixture containing both ID and OOD data. %Although lacking a formal proof for PAC learnability under these conditions, we support our approach with compelling empirical evidence. Further empirical evidence can also be found in \cite{Katz-Habitats-ICML2022}.
\revone, \revthree, \revfour express concerns about assumptions in the PLOSCOD algorithm. %In \cref{sec:pac_learnability}, we demonstrate that, without assumptions about OOD data and given only ID data, solving the SCOD problem is infeasible. 
In \cref{thm:CorrectedSigmoid}, we assume the existence of a feature map $\phi(x)$ which renders the data normally distributed. The assumption is not necessary but is sufficient. %Though the assumption appears strong, in our experiments, we reuse features learned by the ID classifier $h(x)$ transformed only with a single layer. This might not meet the assumption, yet the algorithm performs well. 
While acknowledging the reviewers' point, our current approach is supported by strong empirical results. It is noteworthy that most contemporary binary classifiers implicitly assume normally distributed data by using the sigmoid function in the final layer. \revthree questions the learnability of $\pi_O$ in \cref{equ:gCorrection}. It is crucial to distinguish between the probability distribution $p_O(x)$, and the prior probability $\pi_O$; a single number. This single number scales the entire distribution $p_O(x)$. Consequently, we contest the claim that different combinations of $\pi_O$ and $p_O(x)$, with fixed $p_I(x)$, can yield the same mixture $p_M(x)$. \revone raises questions about \cref{equ:gCorrection}. In theory, \cref{equ:gCorrection} holds. However, we require good estimates of $\pi_O$ and the posterior $p(z\,|\,x)$ to estimate $g(x)$. \revone further raises questions about the mixture coefficient $\pi_O$, see \cref{equ:IDvsUnlabMixture}, claiming that the method is only applicable if $\pi_O$ is known. We disagree; samples can be obtained without knowing the distribution or prior. Value of $\pi_O$ is then estimated from the mixture, see lines 345-360.%$\hat\pi_O$ in %\cref{equ:pluginLratio}.

\boldparagraph{PLOSCOD Mixture}
\hspace{-0.5em}\revthree, \revfour point out that the approach should be validated with varying mixture coefficient $\pi_O$, see \cref{equ:IDvsUnlabMixture}. \revfive asks a related question about the limitations of the PLOSCOD algorithm. For further validation of the practicality of the PLOSCOD algorithm, it would be useful to repeat the experiment with many different mixtures; varying the $\pi_O$. %Investigating the algorithm's performance under extreme conditions, e.g., $\pi_O \approx \nicefrac{1}{1000}$ is an insightful avenue for further experiments. 
With $\pi_O \approx 0$ the method would likely fail, as it would be difficult to estimate $p_O(x)$ using $p(z=M\,|\,x)$. However, we remain confident that our method is well-motivated and effective when $\pi_O \approx 0.5$.%, as evidenced by substantial results.

\boldparagraph{SCOD Motivation}
\hspace{-0.5em}\revtwo and \revfour inquire about the significance of SCOD, and ask for clarification of \cref{def:SCOD}. The motivation for detecting OOD samples is to reject them so their impact on the quality of predictions is reduced. However, some ID samples end up rejected as well. The tasks of selective classification (SC) and OOD detection (OODD) are therefore closely related. Our formulation of the SCOD problem is an extension, addressing both tasks simultaneously. The objective function incorporates two terms \begin{enumerate*}[label=(\roman*),before=\unskip{ }, itemjoin={{, }}, itemjoin*={{, and }}] 
\item $\Rsel(h,c)$ assesses model performance on accepted ID samples (using task-specific loss)
\item $\fpr(c)$ evaluates the portion of incorrectly accepted OOD samples. 
\end{enumerate*}
Relative importance is assigned to the SC and OODD sub-tasks by $\alpha$. Please refer to \cite{Xia-SIRC-ACCV2022, Cen-Devil-ICLR2023, Narasimhan-Plugin-Arxiv2023} for further information on the SCOD problem.

\boldparagraph{SIRC}
\hspace{-0.5em}We apologize to \revthree for our unclear wording regarding the optimal scores. %We want to clarify that 
We do not claim $s_1=r(x)$ and $s_2=g(x)$ to be scores resulting in the best performance of SIRC. We claim that the optimal solution to the SCOD problem involves a linear combination of \begin{enumerate*}[label=(\roman*),before=\unskip{ }, itemjoin={{, }}, itemjoin*={{, and }}]
    \item $r(x)$: optimal solution for SC, minimizing AuRC
    \item $g(x)$: optimal solution for OODD, maximizing AuROC.
\end{enumerate*} 
%We anticipate ongoing advancements in SC and OODD to lead to better approximations of the scores $r(x)$ and $g(x)$.% Consequently, we argue that as these methods progress, the linear combination will increasingly outperform SIRC.

\boldparagraph{Evaluation Metrics}
\hspace{-0.5em}\revtwo is correct that we define three metrics, \cref{ssec:evaluation_metrics}, but only show AuSRT in the paper. Others are shown in the Appendix. AuRC and AuROC are standard metrics for SC and OODD. AuSRT directly addresses the SCOD objective. %By including all three metrics in the Appendix, we assess whether some methods excel in both SC and OODD simultaneously. 
Currently, single-score methods tend to address either SC or OODD; but not both at the same time. The SCOD problem addresses both tasks at the same time. %Further, by combining a score $s_1(x)$ which performs well for SC (low AuRC) with a score $s_2(x)$ which performs well for OODD (high AuROC), we obtain a score which performs well for SCOD (low AuSRT).


\boldparagraph{Distribution Shift}
\hspace{-0.5em}\revfour raises questions about PLOSCOD's robustness to distribution shift. We consider a scenario where the OOD distribution remains consistent between training and test time. Nevertheless, the robustness to distribution shift is only contingent on the relationship between $p_O(x)$ during training and at the test time.

\boldparagraph{Computational Complexity}
\hspace{-0.5em}\revfive inquired about the computational complexity of the algorithm. The complexity aligns with learning the ID classifier $h(x)$ and a binary classifier for the posterior $p(z\,|\,x)$, e.g., using standard neural networks.

==> cifar100_posthoc.tex <==

%\setlength{\tabcolsep}{2pt}

\begin{table}[htbp]
\centering
\caption{The mean and standard deviation over 3-folds of metrics defined in \cref{ssec:evaluation_metrics} shown in \% points for selective classifiers constructed from a CIFAR-100 ID classifier $h(x)$ and selectors $c(x)=\leftbb s(x)\leq \lambda \rightbb$ for a representative sample of single-scores $s(x)$. Results are shown for in-distribution CIFAR-100 using a relative cost of $\alpha=0.5$. The best results are marked in bold, with the second best underlined.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll||c||c|c||c|c||c|c||c|c||c|c||c|c}
\multicolumn{2}{c||}{\multirow{2}{*}{\backslashbox{\it \footnotesize Score}{\it \footnotesize Dataset}}} & ID cifar100 & \multicolumn{2}{c||}{ cifar10} & \multicolumn{2}{c||}{ mnist} & \multicolumn{2}{c||}{ places365} & \multicolumn{2}{c||}{ svhn} & \multicolumn{2}{c||}{ textures} & \multicolumn{2}{c}{ tin}\\
& & \footnotesize AuRC$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ \\ \hline
\multirow{10}{*}{\rotatebox{90}{\bf Single Score}} 
& ASH 
& $8.34 \pm 0.20$ & $76.48 \pm 0.30$ & $15.93 \pm 0.24$ & $77.23 \pm 0.46$ & $15.56 \pm 0.13$ & $78.76 \pm 0.16$ & $14.79 \pm 0.05$ & $\mathbf{85.60 \pm 1.40}$ & $\mathbf{11.37 \pm 0.60}$ & $80.72 \pm 0.70$ & $13.81 \pm 0.25$ & $79.92 \pm 0.20$ & $14.21 \pm 0.17$
\\ \cline{2-15}
&  EBO            
& $7.83 \pm 0.06$ & $\underline{79.05 \pm 0.11}$ & $14.39 \pm 0.07$ & $79.18 \pm 1.37$ & $14.33 \pm 0.67$ & $79.52 \pm 0.23$ & $14.16 \pm 0.13$ & $82.03 \pm 1.74$ & $12.90 \pm 0.90$ & $78.35 \pm 0.83$ & $14.74 \pm 0.45$ & $82.76 \pm 0.08$ & $12.54 \pm 0.04$
\\ \cline{2-15}
&  GradNorm            
& $14.17 \pm 0.18$ & $70.32 \pm 0.20$ & $21.92 \pm 0.16$ & $65.35 \pm 1.12$ & $24.41 \pm 0.48$ & $69.69 \pm 0.17$ & $22.24 \pm 0.14$ & $76.95 \pm 4.73$ & $18.61 \pm 2.40$ & $64.58 \pm 0.13$ & $24.79 \pm 0.15$ & $69.95 \pm 0.79$ & $22.11 \pm 0.38$
\\ \cline{2-15}
&  KNN         
& $\underline{7.28 \pm 0.12}$ & $77.02 \pm 0.25$ & $15.13 \pm 0.08$ & $\underline{82.36 \pm 1.52}$ & $\underline{12.46 \pm 0.79}$ & $79.43 \pm 0.47$ & $13.93 \pm 0.18$ & $\underline{84.15 \pm 1.09}$ & $\underline{11.57 \pm 0.48}$ & $\underline{83.66 \pm 0.83}$ & $\underline{11.81 \pm 0.44}$ & $\mathbf{83.34 \pm 0.16}$ & $\mathbf{11.97 \pm 0.07}$
\\ \cline{2-15}
&  MLS              
& $7.59 \pm 0.07$ & $\mathbf{79.21 \pm 0.10}$ & $\underline{14.19 \pm 0.08}$ & $78.91 \pm 1.47$ & $14.34 \pm 0.72$ & $\underline{79.75 \pm 0.24}$ & $13.92 \pm 0.14$ & $81.65 \pm 1.49$ & $12.97 \pm 0.78$ & $78.39 \pm 0.84$ & $14.60 \pm 0.46$ & $\underline{82.90 \pm 0.05}$ & $12.35 \pm 0.05$
\\ \cline{2-15}
& MSP
& $\mathbf{6.19 \pm 0.12}$ & $78.47 \pm 0.07$ & $\mathbf{13.86 \pm 0.09}$ & $76.08 \pm 1.86$ & $15.06 \pm 0.93$ & $79.22 \pm 0.29$ & $\mathbf{13.49 \pm 0.16}$ & $78.42 \pm 0.89$ & $13.89 \pm 0.51$ & $77.32 \pm 0.71$ & $14.44 \pm 0.41$ & $82.07 \pm 0.17$ & $\underline{12.06 \pm 0.13}$
\\ \cline{2-15}
&  ODIN              
& $8.13 \pm 0.02$ & $78.18 \pm 0.14$ & $14.98 \pm 0.07$ & $\mathbf{83.79 \pm 1.31}$ & $\mathbf{12.17 \pm 0.64}$ & $79.45 \pm 0.26$ & $14.34 \pm 0.14$ & $74.54 \pm 0.76$ & $16.80 \pm 0.39$ & $79.33 \pm 1.08$ & $14.40 \pm 0.55$ & $81.63 \pm 0.08$ & $13.25 \pm 0.04$
\\ \cline{2-15}
&  ReAct              
& $7.66 \pm 0.02$ & $78.65 \pm 0.05$ & $14.50 \pm 0.02$ & $78.37 \pm 1.59$ & $14.65 \pm 0.79$ & $\mathbf{80.03 \pm 0.11}$ & $\underline{13.82 \pm 0.06}$ & $83.01 \pm 0.97$ & $12.33 \pm 0.48$ & $80.15 \pm 0.46$ & $13.76 \pm 0.23$ & $82.88 \pm 0.08$ & $12.39 \pm 0.04$
\\ \cline{2-15}
& VIM
& $8.79 \pm 0.18$ & $72.21 \pm 0.41$ & $18.29 \pm 0.21$ & $81.89 \pm 1.02$ & $13.45 \pm 0.59$ & $75.85 \pm 0.37$ & $16.47 \pm 0.10$ & $83.14 \pm 3.71$ & $12.83 \pm 1.77$ & $\mathbf{85.91 \pm 0.78}$ & $\mathbf{11.44 \pm 0.46}$ & $77.76 \pm 0.16$ & $15.52 \pm 0.13$
\\ 
%\hline
%& \Algo{} LR 
%& 
%\\ 
%\cline{2-15}
%&  Clean LR
%& 
%\\ \cline{2-15}
\end{tabular}
}

\end{table}

%\setlength{\tabcolsep}{6pt}

==> cifar10_posthoc.tex <==

%\setlength{\tabcolsep}{2pt}

\begin{table}[htbp]
\centering
\caption{The mean and standard deviation over 3-folds of metrics defined in \cref{ssec:evaluation_metrics} shown in \% points for selective classifiers constructed from a CIFAR-10 ID classifier $h(x)$ and selectors $c(x)=\leftbb s(x)\leq \lambda \rightbb$ for a representative sample of single-scores $s(x)$. Results are shown for in-distribution CIFAR-10 using a relative cost of $\alpha=0.5$. The best results are marked in bold, with the second best underlined.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll||c||c|c||c|c||c|c||c|c||c|c||c|c}
\multicolumn{2}{c||}{\multirow{2}{*}{\backslashbox{\it \footnotesize Score}{\it \footnotesize Dataset}}} & ID cifar10 & \multicolumn{2}{c||}{ cifar100} & \multicolumn{2}{c||}{ mnist} & \multicolumn{2}{c||}{ places365} & \multicolumn{2}{c||}{ svhn} & \multicolumn{2}{c||}{ textures} & \multicolumn{2}{c}{ tin}\\
& & \footnotesize AuRC$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ & \footnotesize AuROC$\uparrow$ & \footnotesize AuSRT$\downarrow$ \\ \hline
\multirow{10}{*}{\rotatebox{90}{\bf Single Score}} 
& ASH 
& $1.84 \pm 0.27$ & $74.11 \pm 1.55$ & $13.87 \pm 0.89$ & $83.16 \pm 4.66$ & $9.34 \pm 2.35$ & $79.89 \pm 3.69$ & $10.97 \pm 1.71$ & $73.46 \pm 6.41$ & $14.19 \pm 3.28$ & $77.45 \pm 2.39$ & $12.20 \pm 1.33$ & $76.44 \pm 0.61$ & $12.70 \pm 0.44$
\\ \cline{2-15}
&  EBO            
& $0.90 \pm 0.10$ & $86.36 \pm 0.58$ & $7.27 \pm 0.33$ & $94.32 \pm 2.53$ & $3.29 \pm 1.22$ & $89.25 \pm 0.78$ & $5.82 \pm 0.35$ & $91.79 \pm 0.98$ & $4.56 \pm 0.45$ & $89.47 \pm 0.70$ & $5.72 \pm 0.40$ & $88.80 \pm 0.36$ & $6.05 \pm 0.22$
\\ \cline{2-15}
&  GradNorm            
& $3.89 \pm 0.38$ & $54.43 \pm 1.59$ & $24.73 \pm 0.92$ & $63.72 \pm 7.37$ & $20.08 \pm 3.54$ & $60.50 \pm 5.33$ & $21.69 \pm 2.47$ & $53.91 \pm 6.36$ & $24.99 \pm 3.23$ & $52.07 \pm 4.09$ & $25.91 \pm 2.23$ & $55.37 \pm 0.41$ & $24.26 \pm 0.39$
\\ \cline{2-15}
&  KNN         
& $\mathbf{0.56 \pm 0.04}$ & $\mathbf{89.73 \pm 0.14}$ & $\mathbf{5.41 \pm 0.09}$ & $94.26 \pm 0.38$ & $3.15 \pm 0.17$ & $\mathbf{91.77 \pm 0.23}$ & $\mathbf{4.40 \pm 0.11}$ & $\underline{92.67 \pm 0.30}$ & $\underline{3.94 \pm 0.13}$ & $\underline{93.16 \pm 0.24}$ & $\underline{3.70 \pm 0.14}$ & $\mathbf{91.56 \pm 0.26}$ & $\mathbf{4.50 \pm 0.15}$
\\ \cline{2-15}
&  MLS              
& $0.89 \pm 0.10$ & $86.31 \pm 0.59$ & $7.29 \pm 0.33$ & $94.15 \pm 2.48$ & $3.37 \pm 1.19$ & $89.14 \pm 0.76$ & $5.87 \pm 0.34$ & $91.69 \pm 0.94$ & $4.60 \pm 0.43$ & $89.41 \pm 0.71$ & $5.74 \pm 0.41$ & $88.72 \pm 0.36$ & $6.08 \pm 0.23$
\\ \cline{2-15}
& MSP
& $\underline{0.60 \pm 0.03}$ & $87.19 \pm 0.33$ & $6.70 \pm 0.18$ & $92.63 \pm 1.57$ & $3.98 \pm 0.77$ & $88.92 \pm 0.47$ & $5.84 \pm 0.22$ & $91.46 \pm 0.40$ & $4.57 \pm 0.19$ & $89.89 \pm 0.71$ & $5.36 \pm 0.37$ & $88.87 \pm 0.19$ & $5.86 \pm 0.11$
\\ \cline{2-15}
&  ODIN              
& $1.23 \pm 0.22$ & $82.18 \pm 1.87$ & $9.53 \pm 1.04$ & $\mathbf{95.24 \pm 1.96}$ & $\mathbf{3.00 \pm 0.91}$ & $85.07 \pm 1.24$ & $8.08 \pm 0.69$ & $84.58 \pm 0.77$ & $8.33 \pm 0.43$ & $86.94 \pm 2.26$ & $7.15 \pm 1.24$ & $83.55 \pm 1.84$ & $8.84 \pm 1.03$
\\ \cline{2-15}
&  ReAct              
& $0.86 \pm 0.11$ & $85.93 \pm 0.83$ & $7.46 \pm 0.46$ & $92.81 \pm 3.03$ & $4.02 \pm 1.49$ & $\underline{90.35 \pm 0.78}$ & $\underline{5.26 \pm 0.34}$ & $89.12 \pm 3.19$ & $5.87 \pm 1.59$ & $89.38 \pm 1.49$ & $5.74 \pm 0.80$ & $88.29 \pm 0.44$ & $6.29 \pm 0.28$
\\ \cline{2-15}
%&  Residual           
%& $4.34 \pm 0.34$ & $52.17 \pm 0.17$ & $0.00 \pm 0.00$ & $52.17 \pm 0.17$ & $0.00 \pm 0.00$ & $52.17 \pm 0.17$ & $0.00 \pm 0.00$ & $52.17 \pm 0.17$ & $0.00 \pm 0.00$ & $52.17 \pm 0.17$ & $0.00 \pm 0.00$ & $52.17 \pm 0.17$ & $0.00 \pm 0.00$
% \\ \cline{2-15}
&  VIM
& $0.79 \pm 0.05$ & $\underline{87.75 \pm 0.28}$ & $\underline{6.52 \pm 0.16}$ & $\underline{94.76 \pm 0.38}$ & $\underline{3.02 \pm 0.19}$ & $89.49 \pm 0.39$ & $5.65 \pm 0.22$ & $\mathbf{94.51 \pm 0.48}$ & $\mathbf{3.14 \pm 0.22}$ & $\mathbf{95.16 \pm 0.34}$ & $\mathbf{2.82 \pm 0.19}$ & $\underline{89.62 \pm 0.33}$ & $\underline{5.59 \pm 0.19}$
\\ 
%\hline
%& \Algo{} LR 
%& 
%\\ 
%\cline{2-15}
%&  Clean LR
%& 
%\\ \cline{2-15}
\end{tabular}
}
\end{table}

%\setlength{\tabcolsep}{6pt}

==> imagenet_softmax.tex <==
\begin{table*}[]
\centering
\caption{TODO: Imagenet. Binary softmax. Clean OOD data. Results show Area Under SCOD Risk $\downarrow$ in \% points. Beta = 0.5.}
\begin{tabular}{l|c|c|c|c|c}
\backslashbox{\it Score}{\it Dataset} & ssb\_hard & ninco & inaturalist & textures & openimage\_o\\ \hline
SIRC             & \underline{6.82} & \underline{6.66} & \underline{5.52} & \underline{10.27} & \underline{6.86} \\ \hline
Linear           & \bf5.81 & \bf6.60 & \bf4.04 & \bf4.41 & \bf6.05 \\
\hline \hline
MSP              & 17.47 & 13.59 & 9.35 & 12.15 & 11.05 \\ \hline
Likelihood Ratio & 13.90 & 13.95 & 11.25 & 12.15 & 13.87 \\
\end{tabular}
\end{table*}
